Genomic Region Detection via Spatial Convex Clustering

Several modern genomic technologies, such as DNA-Methylation arrays, measure spatially registered probes that number in the hundreds of thousands across multiplechromosomes. The measured probes are by themselves less interesting scientifically; instead scientists seek to discover biologically interpretable genomic regions comprised of contiguous groups of probes which may act as biomarkers of disease or serve as a dimension-reducing pre-processing step for downstream analyses. In this paper, we introduce an unsupervised feature learning technique which maps technological units (probes) to biological units (genomic regions) that are common across all subjects. We use ideas from fusion penalties and convex clustering to introduce a method for Spatial Convex Clustering, or SpaCC. Our method is specifically tailored to detecting multi-subject regions of methylation, but we also test our approach on the well-studied problem of detecting segments of copy number variation. We formulate our method as a convex optimization problem, develop a massively parallelizable algorithm to find its solution, and introduce automated approaches for handling missing values and determining tuning parameters. Through simulation studies based on real methylation and copy number variation data, we show that SpaCC exhibits significant performance gains relative to existing methods. Finally, we illustrate SpaCC's advantages as a pre-processing technique that reduces large-scale genomics data into a smaller number of genomic regions through several cancer epigenetics case studies on subtype discovery, network estimation, and epigenetic-wide association.

==> SpaCCPaper <==
@article{tseng1991applications,
  title={Applications of a splitting algorithm to decomposition in convex programming and variational inequalities},
  author={Tseng, Paul},
  journal={SIAM Journal on Control and Optimization},
  volume={29},
  number={1},
  pages={119--138},
  year={1991},
  publisher={SIAM}
}
@article{mazumder2010spectral,
  title={Spectral regularization algorithms for learning large incomplete matrices},
  author={Mazumder, Rahul and Hastie, Trevor and Tibshirani, Robert},
  journal={The Journal of Machine Learning Research},
  volume={11},
  pages={2287--2322},
  year={2010},
  publisher={JMLR. org}
}
@article{chi2016convex,
  title={Convex biclustering},
  author={Chi, Eric C and Allen, Genevera I and Baraniuk, Richard G},
  journal={Biometrics},
  year={2016},
  publisher={Wiley Online Library}
}

@book{wagner2007comparing,
  title={Comparing clusterings: an overview},
  author={Wagner, Silke and Wagner, Dorothea},
  year={2007},
  publisher={Universit{\"a}t Karlsruhe, Fakult{\"a}t f{\"u}r Informatik Karlsruhe}
}
@article{wold1978cross,
  title={Cross-validatory estimation of the number of components in factor and principal components models},
  author={Wold, Svante},
  journal={Technometrics},
  volume={20},
  number={4},
  pages={397--405},
  year={1978},
  publisher={Taylor \& Francis}
}
@article{olshen2004circular,
  title={Circular binary segmentation for the analysis of array-based DNA copy number data},
  author={Olshen, Adam B and Venkatraman, ES and Lucito, Robert and Wigler, Michael},
  journal={Biostatistics},
  volume={5},
  number={4},
  pages={557--572},
  year={2004},
  publisher={Biometrika Trust}
}
@article{zhang2013package,
  title={Package 'CNTools'},
  author={Zhang, Jianhua and Zhang, Maintainer J and biocViews Microarray, CopyNumberVariants},
  year={2013}
}
@article{seshan2011dnacopy,
  title={DNAcopy: DNA copy number data analysis},
  author={Seshan, Venkatraman E and Olshen, Adam},
  journal={R package version},
  volume={1},
  number={1},
  year={2011}
}
@article{venkatraman2007faster,
  title={A faster circular binary segmentation algorithm for the analysis of array CGH data},
  author={Venkatraman, ES and Olshen, Adam B},
  journal={Bioinformatics},
  volume={23},
  number={6},
  pages={657--663},
  year={2007},
  publisher={Oxford Univ Press}
}
@article{friedman2008sparse,
  title={Sparse inverse covariance estimation with the graphical lasso},
  author={Friedman, Jerome and Hastie, Trevor and Tibshirani, Robert},
  journal={Biostatistics},
  volume={9},
  number={3},
  pages={432--441},
  year={2008},
  publisher={Biometrika Trust}
}
@article{shoemaker2010allele,
  title={Allele-specific methylation is prevalent and is contributed by CpG-SNPs in the human genome},
  author={Shoemaker, Robert and Deng, Jie and Wang, Wei and Zhang, Kun},
  journal={Genome research},
  volume={20},
  number={7},
  pages={883--889},
  year={2010},
  publisher={Cold Spring Harbor Lab}
}
@article{yu2015association,
  title={Association of brain DNA methylation in SORL1, ABCA7, HLA-DRB5, SLC24A4, and BIN1 with pathological diagnosis of Alzheimer disease},
  author={Yu, Lei and Chibnik, Lori B and Srivastava, Gyan P and Pochet, Nathalie and Yang, Jingyun and Xu, Jishu and Kozubek, James and Obholzer, Nikolaus and Leurgans, Sue E and Schneider, Julie A and others},
  journal={JAMA neurology},
  volume={72},
  number={1},
  pages={15--24},
  year={2015},
  publisher={American Medical Association}
}
@article{king2003breast,
  title={Breast and ovarian cancer risks due to inherited mutations in BRCA1 and BRCA2},
  author={King, Mary-Claire and Marks, Joan H and Mandell, Jessica B and others},
  journal={Science},
  volume={302},
  number={5645},
  pages={643--646},
  year={2003},
  publisher={American Association for the Advancement of Science}
}
@article{antoniou2003average,
  title={Average risks of breast and ovarian cancer associated with BRCA1 or BRCA2 mutations detected in case series unselected for family history: a combined analysis of 22 studies},
  author={Antoniou, Anthony and Pharoah, PDP and Narod, Steven and Risch, Harvey A and Eyfjord, Jorunn E and Hopper, JL and Loman, Niklas and Olsson, H{\aa}kan and Johannsson, O and Borg, {\AA}ke and others},
  journal={The American Journal of Human Genetics},
  volume={72},
  number={5},
  pages={1117--1130},
  year={2003},
  publisher={Elsevier}
}
@article{goldstein2014fast,
  title={Fast alternating direction optimization methods},
  author={Goldstein, Tom and O'Donoghue, Brendan and Setzer, Simon and Baraniuk, Richard},
  journal={SIAM Journal on Imaging Sciences},
  volume={7},
  number={3},
  pages={1588--1623},
  year={2014},
  publisher={SIAM}
}
@ARTICLE{ChiLan2014a, 
 author = {Eric C. Chi and Kenneth Lange}, 
 title = {Splitting Methods for Convex Clustering}, 
 journal = {Journal of Computational and Graphical Statistics}, 
 note = {In press}, 
 url = {http://dx.doi.org/10.1080/10618600.2014.948181},
 doi = {10.1080/10618600.2014.948181} 
}
@article{eckhardt2006dna,
  title={DNA methylation profiling of human chromosomes 6, 20 and 22},
  author={Eckhardt, Florian and Lewin, Joern and Cortese, Rene and Rakyan, Vardhman K and Attwood, John and Burger, Matthias and Burton, John and Cox, Tony V and Davies, Rob and Down, Thomas A and others},
  journal={Nature genetics},
  volume={38},
  number={12},
  pages={1378--1385},
  year={2006},
  publisher={Nature Publishing Group}
}
@article{redon2006global,
  title={Global variation in copy number in the human genome},
  author={Redon, Richard and Ishikawa, Shumpei and Fitch, Karen R and Feuk, Lars and Perry, George H and Andrews, T Daniel and Fiegler, Heike and Shapero, Michael H and Carson, Andrew R and Chen, Wenwei and others},
  journal={nature},
  volume={444},
  number={7118},
  pages={444--454},
  year={2006},
  publisher={Nature Publishing Group}
}
@article{brennan2013somatic,
  title={The somatic genomic landscape of glioblastoma},
  author={Brennan, Cameron W and Verhaak, Roel GW and McKenna, Aaron and Campos, Benito and Noushmehr, Houtan and Salama, Sofie R and Zheng, Siyuan and Chakravarty, Debyani and Sanborn, J Zachary and Berman, Samuel H and others},
  journal={Cell},
  volume={155},
  number={2},
  pages={462--477},
  year={2013},
  publisher={Elsevier}
}
@article{ogino2008cohort,
  title={A cohort study of tumoral LINE-1 hypomethylation and prognosis in colon cancer},
  author={Ogino, Shuji and Nosho, Katsuhiko and Kirkner, Gregory J and Kawasaki, Takako and Chan, Andrew T and Schernhammer, Eva S and Giovannucci, Edward L and Fuchs, Charles S},
  journal={Journal of the National Cancer Institute},
  volume={100},
  number={23},
  pages={1734--1738},
  year={2008},
  publisher={Oxford University Press}
}
@article{hsiung2007global,
  title={Global DNA methylation level in whole blood as a biomarker in head and neck squamous cell carcinoma},
  author={Hsiung, Debra Ting and Marsit, Carmen J and Houseman, E Andres and Eddy, Karen and Furniss, C Sloane and McClean, Michael D and Kelsey, Karl T},
  journal={Cancer Epidemiology Biomarkers \& Prevention},
  volume={16},
  number={1},
  pages={108--114},
  year={2007},
  publisher={AACR}
}
@article{meinshausen2009lasso,
  title={Lasso-type recovery of sparse representations for high-dimensional data},
  author={Meinshausen, Nicolai and Yu, Bin},
  journal={The Annals of Statistics},
  pages={246--270},
  year={2009},
  publisher={JSTOR}
}
@article{sebat2007strong,
  title={Strong association of de novo copy number mutations with autism},
  author={Sebat, Jonathan and Lakshmi, B and Malhotra, Dheeraj and Troge, Jennifer and Lese-Martin, Christa and Walsh, Tom and Yamrom, Boris and Yoon, Seungtai and Krasnitz, Alex and Kendall, Jude and others},
  journal={Science},
  volume={316},
  number={5823},
  pages={445--449},
  year={2007},
  publisher={American Association for the Advancement of Science}
}
@article{bergamaschi2006distinct,
  title={Distinct patterns of DNA copy number alteration are associated with different clinicopathological features and gene-expression subtypes of breast cancer},
  author={Bergamaschi, Anna and Kim, Young H and Wang, Pei and S{\o}rlie, Therese and Hernandez-Boussard, Tina and Lonning, Per E and Tibshirani, Robert and B{\o}rresen-Dale, Anne-Lise and Pollack, Jonathan R},
  journal={Genes, Chromosomes and Cancer},
  volume={45},
  number={11},
  pages={1033--1040},
  year={2006},
  publisher={Wiley Online Library}
}
@article{baylin2001aberrant,
  title={Aberrant patterns of DNA methylation, chromatin formation and gene expression in cancer},
  author={Baylin, Stephen B and Esteller, Manel and Rountree, Michael R and Bachman, Kurtis E and Schuebel, Kornel and Herman, James G},
  journal={Human molecular genetics},
  volume={10},
  number={7},
  pages={687--692},
  year={2001},
  publisher={Oxford Univ Press}
}
@article{hunter2004tutorial,
  title={A tutorial on MM algorithms},
  author={Hunter, David R and Lange, Kenneth},
  journal={The American Statistician},
  volume={58},
  number={1},
  pages={30--37},
  year={2004},
  publisher={Taylor \& Francis}
}
@article{kobayashi2011dna,
  title={DNA methylation profiling reveals novel biomarkers and important roles for DNA methyltransferases in prostate cancer},
  author={Kobayashi, Yuya and Absher, Devin M and Gulzar, Zulfiqar G and Young, Sarah R and McKenney, Jesse K and Peehl, Donna M and Brooks, James D and Myers, Richard M and Sherlock, Gavin},
  journal={Genome research},
  volume={21},
  number={7},
  pages={1017--1027},
  year={2011},
  publisher={Cold Spring Harbor Lab}
}
@article{hannum2013genome,
  title={Genome-wide methylation profiles reveal quantitative views of human aging rates},
  author={Hannum, Gregory and Guinney, Justin and Zhao, Ling and Zhang, Li and Hughes, Guy and Sadda, SriniVas and Klotzle, Brandy and Bibikova, Marina and Fan, Jian-Bing and Gao, Yuan and others},
  journal={Molecular cell},
  volume={49},
  number={2},
  pages={359--367},
  year={2013},
  publisher={Elsevier}
}
@article{meinshausen2010stability,
  title={Stability selection},
  author={Meinshausen, Nicolai and B{\"u}hlmann, Peter},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={72},
  number={4},
  pages={417--473},
  year={2010},
  publisher={Wiley Online Library}
}
@article{eisen1998cluster,
  title={Cluster analysis and display of genome-wide expression patterns},
  author={Eisen, Michael B and Spellman, Paul T and Brown, Patrick O and Botstein, David},
  journal={Proceedings of the National Academy of Sciences},
  volume={95},
  number={25},
  pages={14863--14868},
  year={1998},
  publisher={National Acad Sciences}
}
@article{liu2009copy,
  title={Copy number analysis indicates monoclonal origin of lethal metastatic prostate cancer},
  author={Liu, Wennuan and Laitinen, Sari and Khan, Sofia and Vihinen, Mauno and Kowalski, Jeanne and Yu, Guoqiang and Chen, Li and Ewing, Charles M and Eisenberger, Mario A and Carducci, Michael A and others},
  journal={Nature medicine},
  volume={15},
  number={5},
  pages={559--565},
  year={2009},
  publisher={Nature Publishing Group}
}
@article{paz2003systematic,
  title={A systematic profile of DNA methylation in human cancer cell lines},
  author={Paz, Maria F and Fraga, Mario F and Avila, Sonia and Guo, Mingzhou and Pollan, Marina and Herman, James G and Esteller, Manel},
  journal={Cancer research},
  volume={63},
  number={5},
  pages={1114--1121},
  year={2003},
  publisher={AACR}
}
@inproceedings{hocking2011clusterpath,
  title={Clusterpath: an algorithm for clustering using convex fusion penalties},
  author={Hocking, Toby and Vert, Jean-Philippe and Joulin, Armand and Bach, Francis R},
  booktitle={Proceedings of the 28th International Conference on Machine Learning (ICML-11)},
  pages={745--752},
  year={2011}
}
@article{wang2005method,
  title={A method for calling gains and losses in array CGH data},
  author={Wang, Pei and Kim, Young and Pollack, Jonathan and Narasimhan, Balasubramanian and Tibshirani, Robert},
  journal={Biostatistics},
  volume={6},
  number={1},
  pages={45--58},
  year={2005},
  publisher={Biometrika Trust}
}
@article{meilua2007comparing,
  title={Comparing clusterings�an information based distance},
  author={Meil{\u{a}}, Marina},
  journal={Journal of multivariate analysis},
  volume={98},
  number={5},
  pages={873--895},
  year={2007},
  publisher={Elsevier}
}
@article{edgren2011identification,
  title={Identification of fusion genes in breast cancer by paired-end RNA-sequencing},
  author={Edgren, Henrik and Murumagi, Astrid and Kangaspeska, Sara and Nicorici, Daniel and Hongisto, Vesa and Kleivi, Kristine and Rye, Inga H and Nyberg, Sandra and Wolf, Maija and Borresen-Dale, Anne-Lise and others},
  journal={Genome Biol},
  volume={12},
  number={1},
  pages={R6},
  year={2011}
}
@article{vanharanta2013epigenetic,
  title={Epigenetic expansion of VHL-HIF signal output drives multiorgan metastasis in renal cancer},
  author={Vanharanta, Sakari and Shu, Weiping and Brenet, Fabienne and Hakimi, A Ari and Heguy, Adriana and Viale, Agnes and Reuter, Victor E and Hsieh, James JD and Scandura, Joseph M and Massagu{\'e}, Joan},
  journal={Nature medicine},
  volume={19},
  number={1},
  pages={50--56},
  year={2013},
  publisher={Nature Publishing Group}
}
@article{tibshirani2008spatial,
  title={Spatial smoothing and hot spot detection for CGH data using the fused lasso},
  author={Tibshirani, Robert and Wang, Pei},
  journal={Biostatistics},
  volume={9},
  number={1},
  pages={18--29},
  year={2008},
  publisher={Biometrika Trust}
}
@article{nowak2011fused,
  title={A fused lasso latent feature model for analyzing multi-sample aCGH data},
  author={Nowak, Gen and Hastie, Trevor and Pollack, Jonathan R and Tibshirani, Robert},
  journal={Biostatistics},
  pages={kxr012},
  year={2011},
  publisher={Biometrika Trust}
}
@article{bleakley2011group,
  title={The group fused lasso for multiple change-point detection},
  author={Bleakley, Kevin and Vert, Jean-Philippe},
  journal={arXiv preprint arXiv:1106.4199},
  year={2011}
}
@article{baylin2005dna,
  title={DNA methylation and gene silencing in cancer},
  author={Baylin, Stephen B},
  journal={Nature clinical practice Oncology},
  volume={2},
  pages={S4--S11},
  year={2005},
  publisher={Nature Publishing Group}
}
@article{herman1995inactivation,
  title={Inactivation of the CDKN2/p16/MTS1 gene is frequently associated with aberrant DNA methylation in all common human cancers},
  author={Herman, James G and Merlo, Adrian and Mao, LI and Lapidus, Rena G and Issa, Jean-Pierre J and Davidson, Nancy E and Sidransky, David and Baylin, Stephen B},
  journal={Cancer research},
  volume={55},
  number={20},
  pages={4525--4530},
  year={1995},
  publisher={AACR}
}
@article{widschwendter2002dna,
  title={DNA methylation and breast carcinogenesis.},
  author={Widschwendter, Martin and Jones, Peter A},
  journal={Oncogene},
  volume={21},
  number={35},
  pages={5462--5482},
  year={2002}
}
@article{muggerud2010frequent,
  title={Frequent aberrant DNA methylation of ABCB1, FOXC1, PPP2R2B and PTEN in ductal carcinoma in situ and early invasive breast cancer},
  author={Muggerud, Aslaug A and R{\o}nneberg, Jo Anders and W{\"a}rnberg, Fredrik and Botling, Johan and Busato, Florence and Jovanovic, Jovana and Solvang, Hiroko and Bukholm, Ida and B{\o}rresen-Dale, Anne-Lise and Kristensen, Vessela N and others},
  journal={Breast Cancer Research},
  volume={12},
  number={1},
  pages={R3},
  year={2010},
  publisher={BioMed Central Ltd}
}
@article{szyf2004dna,
  title={DNA methylation and breast cancer},
  author={Szyf, Moshe and Pakneshan, Pouya and Rabbani, Shafaat A},
  journal={Biochemical pharmacology},
  volume={68},
  number={6},
  pages={1187--1197},
  year={2004},
  publisher={Elsevier}
}
@article{das2004dna,
  title={DNA methylation and cancer},
  author={Das, Partha M and Singal, Rakesh},
  journal={Journal of clinical oncology},
  volume={22},
  number={22},
  pages={4632--4642},
  year={2004},
  publisher={American Society of Clinical Oncology}
}
@article{esteller2000promoter,
  title={Promoter hypermethylation and BRCA1 inactivation in sporadic breast and ovarian tumors},
  author={Esteller, Manel and Silva, Jose Maria and Dominguez, Gemma and Bonilla, Felix and Matias-Guiu, Xavier and Lerma, Enrique and Bussaglia, Elena and Prat, Jaime and Harkes, I Clara and Repasky, Elizabeth A and others},
  journal={Journal of the National Cancer Institute},
  volume={92},
  number={7},
  pages={564--569},
  year={2000},
  publisher={Oxford University Press}
}
@article{catteau1999methylation,
  title={Methylation of the BRCA1 promoter region in sporadic breast and ovarian cancer: correlation with disease characteristics},
  author={Catteau, Aurelie and Harris, William H and Xu, Chun-Fang and Solomon, Ellen},
  journal={Oncogene},
  volume={18},
  number={11},
  pages={1957--1965},
  year={1999}
}
@article{etemadmoghadam2009integrated,
  title={Integrated genome-wide DNA copy number and expression analysis identifies distinct mechanisms of primary chemoresistance in ovarian carcinomas},
  author={Etemadmoghadam, Dariush and Beroukhim, Rameen and Mermel, Craig and George, Joshy and Getz, Gad and Tothill, Richard and Okamoto, Aikou and Raeder, Maria B and Harnett, Paul and Lade, Stephen and others},
  journal={Clinical Cancer Research},
  volume={15},
  number={4},
  pages={1417--1427},
  year={2009},
  publisher={AACR}
}
@article{anzick1997aib1,
  title={AIB1, a steroid receptor coactivator amplified in breast and ovarian cancer},
  author={Anzick, Sarah L and Kononen, Juha and Walker, Robert L and Azorsa, David O and Tanner, Minna M and Guan, Xin-Yuan and Sauter, Guido and Kallioniemi, Olli-P and Trent, Jeffrey M and Meltzer, Paul S},
  journal={Science},
  volume={277},
  number={5328},
  pages={965--968},
  year={1997},
  publisher={American Association for the Advancement of Science}
}
@article{iwabuchi1995genetic,
  title={Genetic analysis of benign, low-grade, and high-grade ovarian tumors},
  author={Iwabuchi, Hiroshi and Sakamoto, Masaru and Sakunaga, Hotaka and Ma, Yen-Ying and Carcangiu, Maria L and Pinkel, Daniel and Yang-Feng, Teresa L and Gray, Joe W},
  journal={Cancer Research},
  volume={55},
  number={24},
  pages={6172--6180},
  year={1995},
  publisher={AACR}
}

@article{hansen2012bsmooth,
  title={BSmooth: from whole genome bisulfite sequencing reads to differentially methylated regions},
  author={Hansen, Kasper D and Langmead, Benjamin and Irizarry, Rafael A and others},
  journal={Genome Biol},
  volume={13},
  number={10},
  pages={R83},
  year={2012}
}
@article{jaffe2012bump,
  title={Bump hunting to identify differentially methylated regions in epigenetic epidemiology studies},
  author={Jaffe, Andrew E and Murakami, Peter and Lee, Hwajin and Leek, Jeffrey T and Fallin, M Daniele and Feinberg, Andrew P and Irizarry, Rafael A},
  journal={International journal of epidemiology},
  volume={41},
  number={1},
  pages={200--209},
  year={2012},
  publisher={IEA}
}
@article{michels2013recommendations,
  title={Recommendations for the design and analysis of epigenome-wide association studies},
  author={Michels, Karin B and Binder, Alexandra M and Dedeurwaerder, Sarah and Epstein, Charles B and Greally, John M and Gut, Ivo and Houseman, E Andres and Izzi, Benedetta and Kelsey, Karl T and Meissner, Alexander and others},
  journal={Nature methods},
  volume={10},
  number={10},
  pages={949--955},
  year={2013},
  publisher={Nature Publishing Group}
}
@article{bell2012epigenome,
  title={Epigenome-wide scans identify differentially methylated regions for age and age-related phenotypes in a healthy ageing population},
  author={Bell, Jordana T and Tsai, Pei-Chien and Yang, Tsun-Po and Pidsley, Ruth and Nisbet, James and Glass, Daniel and Mangino, Massimo and Zhai, Guangju and Zhang, Feng and Valdes, Ana and others},
  journal={PLoS Genet},
  volume={8},
  number={4},
  pages={e1002629},
  year={2012},
  publisher={Public Library of Science}
}
@article{houseman2008model,
  title={Model-based clustering of DNA methylation array data: a recursive-partitioning algorithm for high-dimensional data arising as a mixture of beta distributions},
  author={Houseman, E Andres and Christensen, Brock C and Yeh, Ru-Fang and Marsit, Carmen J and Karagas, Margaret R and Wrensch, Margaret and Nelson, Heather H and Wiemels, Joseph and Zheng, Shichun and Wiencke, John K and others},
  journal={BMC bioinformatics},
  volume={9},
  number={1},
  pages={1},
  year={2008},
  publisher={BioMed Central}
}
@article{langevin2011influence,
  title={The influence of aging, environmental exposures and local sequence features on the variation of DNA methylation in blood},
  author={Langevin, Scott M and Houseman, E Andres and Christensen, Brock C and Wiencke, John K and Nelson, Heather H and Karagas, Margaret R and Marsit, Carmen J and Kelsey, Karl T},
  journal={epigenetics},
  volume={6},
  number={7},
  pages={908--919},
  year={2011},
  publisher={Taylor \& Francis}
}
@article{xu2013epigenome,
  title={Epigenome-wide association study of breast cancer using prospectively collected sister study samples},
  author={Xu, Zongli and Bolick, Sophia CE and DeRoo, Lisa A and Weinberg, Clarice R and Sandler, Dale P and Taylor, Jack A},
  journal={Journal of the National Cancer Institute},
  volume={105},
  number={10},
  pages={694--700},
  year={2013},
  publisher={Oxford University Press}
}
@article{weisenberger2006cpg,
  title={CpG island methylator phenotype underlies sporadic microsatellite instability and is tightly associated with BRAF mutation in colorectal cancer},
  author={Weisenberger, Daniel J and Siegmund, Kimberly D and Campan, Mihaela and Young, Joanne and Long, Tiffany I and Faasse, Mark A and Kang, Gyeong Hoon and Widschwendter, Martin and Weener, Deborah and Buchanan, Daniel and others},
  journal={Nature genetics},
  volume={38},
  number={7},
  pages={787--793},
  year={2006},
  publisher={Nature Publishing Group}
}
@article{ward1963hierarchical,
  title={Hierarchical grouping to optimize an objective function},
  author={Ward Jr, Joe H},
  journal={Journal of the American statistical association},
  volume={58},
  number={301},
  pages={236--244},
  year={1963},
  publisher={Taylor \& Francis}
}
@article{pollack2002microarray,
  title={Microarray analysis reveals a major direct role of DNA copy number alteration in the transcriptional program of human breast tumors},
  author={Pollack, Jonathan R and S{\o}rlie, Therese and Perou, Charles M and Rees, Christian A and Jeffrey, Stefanie S and Lonning, Per E and Tibshirani, Robert and Botstein, David and B{\o}rresen-Dale, Anne-Lise and Brown, Patrick O},
  journal={Proceedings of the National Academy of Sciences},
  volume={99},
  number={20},
  pages={12963--12968},
  year={2002},
  publisher={National Acad Sciences}
}
@article{virmani2002hierarchical,
  title={Hierarchical clustering of lung cancer cell lines using DNA methylation markers},
  author={Virmani, Arvind K and Tsou, Jeffrey A and Siegmund, Kimberly D and Shen, Linda YC and Long, Tiffany I and Laird, Peter W and Gazdar, Adi F and Laird-Offringa, Ite A},
  journal={Cancer Epidemiology Biomarkers \& Prevention},
  volume={11},
  number={3},
  pages={291--297},
  year={2002},
  publisher={AACR}
}
@article{shen2007integrated,
  title={Integrated genetic and epigenetic analysis identifies three different subclasses of colon cancer},
  author={Shen, Lanlan and Toyota, Minoru and Kondo, Yutaka and Lin, E and Zhang, Li and Guo, Yi and Hernandez, Natalie Supunpong and Chen, Xinli and Ahmed, Saira and Konishi, Kazuo and others},
  journal={Proceedings of the National Academy of Sciences},
  volume={104},
  number={47},
  pages={18654--18659},
  year={2007},
  publisher={National Acad Sciences}
}
@article{shi2005tumor,
  title={Tumor classification by tissue microarray profiling: random forest clustering applied to renal cell carcinoma},
  author={Shi, Tao and Seligson, David and Belldegrun, Arie S and Palotie, Aarno and Horvath, Steve},
  journal={Modern Pathology},
  volume={18},
  number={4},
  pages={547--557},
  year={2005},
  publisher={Nature Publishing Group}
}
@article{taylor2008functional,
  title={Functional copy-number alterations in cancer},
  author={Taylor, Barry S and Barretina, Jordi and Socci, Nicholas D and DeCarolis, Penelope and Ladanyi, Marc and Meyerson, Matthew and Singer, Samuel and Sander, Chris},
  journal={PloS one},
  volume={3},
  number={9},
  pages={e3179},
  year={2008},
  publisher={Public Library of Science}
}

@article{boyd2011distributed,
  title={Distributed optimization and statistical learning via the alternating direction method of multipliers},
  author={Boyd, Stephen and Parikh, Neal and Chu, Eric and Peleato, Borja and Eckstein, Jonathan},
  journal={Foundations and Trends{\textregistered} in Machine Learning},
  volume={3},
  number={1},
  pages={1--122},
  year={2011},
  publisher={Now Publishers Inc.}
}
@article{hashimoto2004requirement,
  title={Requirement for Arf6 in breast cancer invasive activities},
  author={Hashimoto, Shigeru and Onodera, Yasuhito and Hashimoto, Ari and Tanaka, Miwa and Hamaguchi, Michinari and Yamada, Atsuko and Sabe, Hisataka},
  journal={Proceedings of the National Academy of Sciences of the United States of America},
  volume={101},
  number={17},
  pages={6647--6652},
  year={2004},
  publisher={National Acad Sciences}
}
@article{malaby2013structural,
  title={Structural basis for membrane recruitment and allosteric activation of cytohesin family Arf GTPase exchange factors},
  author={Malaby, Andrew W and van den Berg, Bert and Lambright, David G},
  journal={Proceedings of the National Academy of Sciences},
  volume={110},
  number={35},
  pages={14213--14218},
  year={2013},
  publisher={National Acad Sciences}
}
@article{morishige2008gep100,
  title={GEP100 links epidermal growth factor receptor signalling to Arf6 activation to induce breast cancer invasion},
  author={Morishige, Masaki and Hashimoto, Shigeru and Ogawa, Eiji and Toda, Yoshinobu and Kotani, Hirokazu and Hirose, Mayumi and Wei, Shumei and Hashimoto, Ari and Yamada, Atsuko and Yano, Hajime and others},
  journal={Nature cell biology},
  volume={10},
  number={1},
  pages={85--92},
  year={2008},
  publisher={Nature Publishing Group}
}
@article{hussain2009dubs,
  title={DUBs and cancer: the role of deubiquitinating enzymes as oncogenes, non-oncogenes and tumor suppressors},
  author={Hussain, Sajjad and Zhang, Ying and Galardy, Paul},
  journal={Cell cycle},
  volume={8},
  number={11},
  pages={1688--1697},
  year={2009},
  publisher={Taylor \& Francis}
}
@article{shao2014adam,
  title={ADAM-12 as a diagnostic marker for the proliferation, migration and invasion in patients with small cell lung cancer},
  author={Shao, Shuhong and Li, Zunling and Gao, Wei and Yu, Guohua and Liu, Dexiang and Pan, Fang},
  journal={PloS one},
  volume={9},
  number={1},
  pages={e85936},
  year={2014},
  publisher={Public Library of Science}
}
@article{repapi2010genome,
  title={Genome-wide association study identifies five loci associated with lung function},
  author={Repapi, Emmanouela and Sayers, Ian and Wain, Louise V and Burton, Paul R and Johnson, Toby and Obeidat, Ma'en and Zhao, Jing Hua and Ramasamy, Adaikalavan and Zhai, Guangju and Vitart, Veronique and others},
  journal={Nature genetics},
  volume={42},
  number={1},
  pages={36--44},
  year={2010},
  publisher={Nature Publishing Group}
}
@article{zenklusen2001mutational,
  title={Mutational and functional analyses reveal that ST7 is a highly conserved tumor-suppressor gene on human chromosome 7q31},
  author={Zenklusen, Jean C and Conti, Claudio J and Green, Eric D},
  journal={Nature genetics},
  volume={27},
  number={4},
  pages={392--398},
  year={2001},
  publisher={Nature Publishing Group}
}
@article{furukawa2005plakophilin,
  title={Plakophilin 3 oncogene as prognostic marker and therapeutic target for lung cancer},
  author={Furukawa, Chiyuki and Daigo, Yataro and Ishikawa, Nobuhisa and Kato, Tatsuya and Ito, Tomoo and Tsuchiya, Eiju and Sone, Saburo and Nakamura, Yusuke},
  journal={Cancer Research},
  volume={65},
  number={16},
  pages={7102--7110},
  year={2005},
  publisher={AACR}
}
@article{zhang2012chimeric,
  title={Chimeric transcript generated by cis-splicing of adjacent genes regulates prostate cancer cell proliferation},
  author={Zhang, Yanmei and Gong, Mei and Yuan, Huiling and Park, Hong G and Frierson, Henry F and Li, Hui},
  journal={Cancer discovery},
  volume={2},
  number={7},
  pages={598--607},
  year={2012},
  publisher={AACR}
}
@article{kelley2010ypel3,
  title={YPEL3, a p53-regulated gene that induces cellular senescence},
  author={Kelley, Kevin D and Miller, Kelly R and Todd, Amber and Kelley, Amy R and Tuttle, Rebecca and Berberich, Steven J},
  journal={Cancer research},
  volume={70},
  number={9},
  pages={3566--3575},
  year={2010},
  publisher={AACR}
}
@article{chen2014epigenetic,
  title={Epigenetic regulation and cancer (Review)},
  author={Chen, QW and Zhu, XY and Li, YY and Meng, ZQ},
  journal={Oncology reports},
  volume={31},
  number={2},
  pages={523--532},
  year={2014},
  publisher={Spandidos Publications}
}
@article{maeda2007transcriptional,
  title={Transcriptional control of lung morphogenesis},
  author={Maeda, Yutaka and Dav{\'e}, Vrushank and Whitsett, Jeffrey A},
  journal={Physiological reviews},
  volume={87},
  number={1},
  pages={219--244},
  year={2007},
  publisher={Am Physiological Soc}
}
@article{borczuk2003non,
  title={Non-small-cell lung cancer molecular signatures recapitulate lung developmental pathways},
  author={Borczuk, Alain C and Gorenstein, Lyall and Walter, Kristin L and Assaad, Adel A and Wang, Liqun and Powell, Charles A},
  journal={The American journal of pathology},
  volume={163},
  number={5},
  pages={1949--1960},
  year={2003},
  publisher={Elsevier}
}
@article{anglim2008identification,
  title={Identification of a panel of sensitive and specific DNA methylation markers for squamous cell lung cancer},
  author={Anglim, Paul P and Galler, Janice S and Koss, Michael N and Hagen, Jeffrey A and Turla, Sally and Campan, Mihaela and Weisenberger, Daniel J and Laird, Peter W and Siegmund, Kimberly D and Laird-Offringa, Ite A},
  journal={Molecular cancer},
  volume={7},
  number={1},
  pages={1},
  year={2008},
  publisher={BioMed Central}
}
@article{mcnerney2013cux1,
  title={CUX1 is a haploinsufficient tumor suppressor gene on chromosome 7 frequently inactivated in acute myeloid leukemia},
  author={McNerney, Megan E and Brown, Christopher D and Wang, Xiaoyue and Bartom, Elizabeth T and Karmakar, Subhradip and Bandlamudi, Chaitanya and Yu, Shan and Ko, Jinkyung and Sandall, Barry P and Stricker, Thomas and others},
  journal={Blood},
  volume={121},
  number={6},
  pages={975--983},
  year={2013},
  publisher={Am Soc Hematology}
}
@article{pacurari2011multi,
  title={Multi-walled carbon nanotube-induced gene expression in the mouse lung: association with lung pathology},
  author={Pacurari, M and Qian, Y and Porter, DW and Wolfarth, M and Wan, Y and Luo, D and Ding, M and Castranova, V and Guo, NL},
  journal={Toxicology and applied pharmacology},
  volume={255},
  number={1},
  pages={18--31},
  year={2011},
  publisher={Elsevier}
}
@article{wan2010hybrid,
  title={Hybrid models identified a 12-gene signature for lung cancer prognosis and chemoresponse prediction},
  author={Wan, Ying-Wooi and Sabbagh, Ebrahim and Raese, Rebecca and Qian, Yong and Luo, Dajie and Denvir, James and Vallyathan, Val and Castranova, Vincent and Guo, Nancy Lan},
  journal={PLoS One},
  volume={5},
  number={8},
  pages={e12222},
  year={2010},
  publisher={Public Library of Science}
}

@article{tsai2009microrna,
  title={MicroRNA-122, a tumor suppressor microRNA that regulates intrahepatic metastasis of hepatocellular carcinoma},
  author={Tsai, Wei-Chih and Hsu, Paul Wei-Che and Lai, Tsung-Ching and Chau, Gar-Yang and Lin, Ching-Wen and Chen, Chun-Ming and Lin, Chien-Der and Liao, Yu-Lun and Wang, Jui-Ling and Chau, Yat-Pang and others},
  journal={Hepatology},
  volume={49},
  number={5},
  pages={1571--1582},
  year={2009},
  publisher={Wiley Online Library}
}
@phdthesis{cao2014zinc,
  title={ZINC FINGER, AN1-TYPE DOMAIN 2A---A NOVEL TARGET FOR LUNG CANCER THERAPY},
  author={Cao, Shuo},
  year={2014},
  school={University of Pittsburgh}
}
@article{miyoshi2008biological,
  title={Biological function of fucosylation in cancer biology},
  author={Miyoshi, Eiji and Moriwaki, Kenta and Nakagawa, Tsutomu},
  journal={Journal of biochemistry},
  volume={143},
  number={6},
  pages={725--729},
  year={2008},
  publisher={Jpn Biochemical Soc}
}
@article{cao2012glycerophosphodiester,
  title={Glycerophosphodiester phosphodiesterase domain containing 5 (GDPD5) expression correlates with malignant choline phospholipid metabolite profiles in human breast cancer},
  author={Cao, Maria D and D{\"o}pkens, Mailin and Krishnamachary, Balaji and Vesuna, Farhad and Gadiya, Mayur M and L{\o}nning, Per E and Bhujwalla, Zaver M and Gribbestad, Ingrid S and Glunde, Kristine},
  journal={NMR in biomedicine},
  volume={25},
  number={9},
  pages={1033--1042},
  year={2012},
  publisher={Wiley Online Library}
}
@article{berretta2010cancer,
  title={Cancer biomarker discovery: the entropic hallmark},
  author={Berretta, Regina and Moscato, Pablo},
  journal={PLoS One},
  volume={5},
  number={8},
  pages={e12262},
  year={2010},
  publisher={Public Library of Science}
}
@article{l2008global,
  title={Global gene expression analysis of early response to chemotherapy treatment in ovarian cancer spheroids},
  author={L'Esp{\'e}rance, Sylvain and Bachvarova, Magdalena and Tetu, Bernard and Mes-Masson, Anne-Marie and Bachvarov, Dimcho},
  journal={BMC genomics},
  volume={9},
  number={1},
  pages={1},
  year={2008},
  publisher={BioMed Central}
}
@article{mathews2010epigenetic,
  title={Epigenetic regulation of CpG promoter methylation in invasive prostate cancer cells},
  author={Mathews, Lesley A and Hurt, Elaine M and Zhang, Xiaohu and Farrar, William L},
  journal={Molecular cancer},
  volume={9},
  number={1},
  pages={1},
  year={2010},
  publisher={BioMed Central}
}
@article{fujitomo2012critical,
  title={Critical function for nuclear envelope protein TMEM209 in human pulmonary carcinogenesis},
  author={Fujitomo, Takashi and Daigo, Yataro and Matsuda, Koichi and Ueda, Koji and Nakamura, Yusuke},
  journal={Cancer research},
  volume={72},
  number={16},
  pages={4110--4118},
  year={2012},
  publisher={AACR}
}
@article{cruickshanks2013expression,
  title={Expression of a large LINE-1-driven antisense RNA is linked to epigenetic silencing of the metastasis suppressor gene TFPI-2 in cancer},
  author={Cruickshanks, Hazel A and Vafadar-Isfahani, Natasha and Dunican, Donncha S and Lee, Andy and Sproul, Duncan and Lund, Jonathan N and Meehan, Richard R and Tufarelli, Cristina},
  journal={Nucleic acids research},
  volume={41},
  number={14},
  pages={6857--6869},
  year={2013},
  publisher={Oxford Univ Press}
}
@article{chen2007immunoglobulin,
  title={Immunoglobulin G expression in carcinomas and cancer cell lines},
  author={Chen, Zhengshan and Gu, Jiang},
  journal={The FASEB Journal},
  volume={21},
  number={11},
  pages={2931--2938},
  year={2007},
  publisher={FASEB}
}
@article{yang2010role,
  title={The role of microRNA in human lung squamous cell carcinoma},
  author={Yang, Ye and Li, Xiaofei and Yang, Qi and Wang, Xiaoping and Zhou, Yongan and Jiang, Tao and Ma, Qunfeng and Wang, Yun-Jie},
  journal={Cancer genetics and cytogenetics},
  volume={200},
  number={2},
  pages={127--133},
  year={2010},
  publisher={Elsevier}
}
@article{giunti2014genome,
  title={Genome-wide copy number analysis in pediatric glioblastoma multiforme},
  author={Giunti, Laura and Pantaleo, Marilena and Sardi, Iacopo and Provenzano, Aldesia and Magi, Alberto and Cardellicchio, Stefania and Castiglione, Francesca and Tattini, Lorenzo and Novara, Francesca and Buccoliero, Anna Maria and others},
  journal={Am J Cancer Res},
  volume={4},
  pages={293--303},
  year={2014}
}
@article{suzuki2008identification,
  title={Identification of SMURF1 as a possible target for 7q21. 3-22.1 amplification detected in a pancreatic cancer cell line by in-house array-based comparative genomic hybridization},
  author={Suzuki, Ayako and Shibata, Tatsuhiro and Shimada, Yutaka and Murakami, Yoshinori and Horii, Akira and Shiratori, Keiko and Hirohashi, Setsuo and Inazawa, Johji and Imoto, Issei},
  journal={Cancer science},
  volume={99},
  number={5},
  pages={986--994},
  year={2008},
  publisher={Wiley Online Library}
}
@article{kwei2011smurf1,
  title={SMURF1 amplification promotes invasiveness in pancreatic cancer},
  author={Kwei, Kevin A and Shain, A Hunter and Bair, Ryan and Montgomery, Kelli and Karikari, Collins A and van de Rijn, Matt and Hidalgo, Manuel and Maitra, Anirban and Bashyam, Murali D and Pollack, Jonathan R},
  journal={PloS one},
  volume={6},
  number={8},
  pages={e23924},
  year={2011},
  publisher={Public Library of Science}
}
@article{xie2011smurf1,
  title={Smurf1 ubiquitin ligase targets Kruppel-like factor KLF2 for ubiquitination and degradation in human lung cancer H1299 cells},
  author={Xie, Ping and Tang, Ying and Shen, Shan and Wang, Yunyan and Xing, Guichun and Yin, Yuxin and He, Fuchu and Zhang, Lingqiang},
  journal={Biochemical and biophysical research communications},
  volume={407},
  number={1},
  pages={254--259},
  year={2011},
  publisher={Elsevier}
}
@article{dhillonbig,
  title={BIG \& QUIC: Sparse Inverse Covariance Estimation for a Million Variables},
  author={Dhillon, Inderjit S}
}
@article{ushijima2005detection,
  title={Detection and interpretation of altered methylation patterns in cancer cells},
  author={Ushijima, Toshikazu},
  journal={Nature Reviews Cancer},
  volume={5},
  number={3},
  pages={223--231},
  year={2005},
  publisher={Nature Publishing Group}
}
@article{hupe2004analysis,
  title={Analysis of array CGH data: from signal ratio to gain and loss of DNA regions},
  author={Hup{\'e}, Philippe and Stransky, Nicolas and Thiery, Jean-Paul and Radvanyi, Fran{\c{c}}ois and Barillot, Emmanuel},
  journal={Bioinformatics},
  volume={20},
  number={18},
  pages={3413--3422},
  year={2004},
  publisher={Oxford Univ Press}
}
@article{lai2005comparative,
  title={Comparative analysis of algorithms for identifying amplifications and deletions in array CGH data},
  author={Lai, Weil R and Johnson, Mark D and Kucherlapati, Raju and Park, Peter J},
  journal={Bioinformatics},
  volume={21},
  number={19},
  pages={3763--3770},
  year={2005},
  publisher={Oxford Univ Press}
}
@article{pinkel1998high,
  title={High resolution analysis of DNA copy number variation using comparative genomic hybridization to microarrays},
  author={Pinkel, Daniel and Segraves, Richard and Sudar, Damir and Clark, Steven and Poole, Ian and Kowbel, David and Collins, Colin and Kuo, Wen-Lin and Chen, Chira and Zhai, Ye and others},
  journal={Nature genetics},
  volume={20},
  number={2},
  pages={207--211},
  year={1998},
  publisher={Nature Publishing Group}
}
@article{jaenisch2003epigenetic,
  title={Epigenetic regulation of gene expression: how the genome integrates intrinsic and environmental signals},
  author={Jaenisch, Rudolf and Bird, Adrian},
  journal={Nature genetics},
  volume={33},
  pages={245--254},
  year={2003},
  publisher={Nature Publishing Group}
}
@article{sato2003frequent,
  title={Frequent hypomethylation of multiple genes overexpressed in pancreatic ductal adenocarcinoma},
  author={Sato, Norihiro and Maitra, Anirban and Fukushima, Noriyoshi and van Heek, N Tjarda and Matsubayashi, Hiroyuki and Iacobuzio-Donahue, Christine A and Rosty, Christophe and Goggins, Michael},
  journal={Cancer Research},
  volume={63},
  number={14},
  pages={4158--4166},
  year={2003},
  publisher={AACR}
}
@article{tibshirani2005sparsity,
  title={Sparsity and smoothness via the fused lasso},
  author={Tibshirani, Robert and Saunders, Michael and Rosset, Saharon and Zhu, Ji and Knight, Keith},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={67},
  number={1},
  pages={91--108},
  year={2005},
  publisher={Wiley Online Library}
}
@article{cancer2011integrated,
  title={Integrated genomic analyses of ovarian carcinoma},
  author={Cancer Genome Atlas Research Network and others},
  journal={Nature},
  volume={474},
  number={7353},
  pages={609--615},
  year={2011},
  publisher={Nature Publishing Group}
}
@Manual{dnacopy,
    title = {DNAcopy: DNA copy number data analysis},
    author = {Venkatraman E. Seshan and Adam Olshen},
    note = {R package version 1.40.0},
}
@Manual{cntools,
    title = {CNTools: Convert segment data into a region by sample matrix to allow for
other high level computational analyses.},
    author = {Jianhua Zhang},
    note = {R package version 1.22.0},
}
@article{cancer2012comprehensive,
  title={Comprehensive molecular portraits of human breast tumours},
  author={Cancer Genome Atlas Network and others},
  journal={Nature},
  volume={490},
  number={7418},
  pages={61--70},
  year={2012},
  publisher={Nature Publishing Group}
}
@article{o2008functional,
  title={Functional genomics identifies ABCC3 as a mediator of taxane resistance in HER2-amplified breast cancer},
  author={O'Brien, Carol and Cavet, Guy and Pandita, Ajay and Hu, Xiaolan and Haydu, Lauren and Mohan, Sankar and Toy, Karen and Rivers, Celina Sanchez and Modrusan, Zora and Amler, Lukas C and others},
  journal={Cancer research},
  volume={68},
  number={13},
  pages={5380--5389},
  year={2008},
  publisher={AACR}
}
@article{mita2007prognostic,
  title={Prognostic significance of insulin-like growth factor binding protein (IGFBP)-4 and IGFBP-5 expression in breast cancer},
  author={Mita, Keiko and Zhang, Zhenhuan and Ando, Yoshiaki and Toyama, Tatsuya and Hamaguchi, Maho and Kobayashi, Shunzo and Hayashi, Shin-ichi and Fujii, Yoshitaka and Iwase, Hirotaka and Yamashita, Hiroko},
  journal={Japanese journal of clinical oncology},
  volume={37},
  number={8},
  pages={575--582},
  year={2007},
  publisher={FPCR}
}
@article{mongroo2011imp,
         title={IMP-1 displays cross-talk with K-Ras and modulates colon cancer cell survival through the novel proapoptotic protein CYFIP2},
         author={Mongroo, Perry S and Noubissi, Felicite K and Cuatrecasas, Miriam and Kalabis, Jiri and King, Catrina E and Johnstone, Cameron N and Bowser, Mark J and Castells, Antoni and Spiegelman, Vladimir S and Rustgi, Anil K},
         journal={Cancer research},
         volume={71},
         number={6},
         pages={2172--2182},
         year={2011},
         publisher={AACR}
}
@article{zhang2015elevated,
         title={Elevated NIBP/TRAPPC9 mediates tumorigenesis of cancer cells through NF$\kappa$B signaling},
         author={Zhang, Yonggang and Liu, Shu and Wang, Hong and Yang, Wensheng and Li, Fang and Yang, Fan and Yu, Daohai and Ramsey, Frederick V and Tuszyski, George P and Hu, Wenhui},
         journal={Oncotarget},
         volume={6},
         number={8},
         pages={6160},
         year={2015},
         publisher={Impact Journals, LLC}
}

@article{taniwaki2006gene,
         title={Gene expression profiles of small-cell lung cancers: molecular signatures of lung cancer},
         author={Taniwaki, Masaya and Daigo, Yataro and Ishikawa, Nobuhisa and Takano, Atsushi and Tsunoda, Tatsuhiko and Yasui, Wataru and Inai, Kouki and Kohno, Nobuoki and Nakamura, Yusuke},
         journal={markers},
         volume={12},
         pages={17},
         year={2006}
}
@article{moriwaki2009deficiency,
         title={Deficiency of GMDS leads to escape from NK cell-mediated tumor surveillance through modulation of TRAIL signaling},
         author={Moriwaki, Kenta and Noda, Katsuhisa and Furukawa, Yoichi and Ohshima, Kenji and Uchiyama, Airi and Nakagawa, Tsutomu and Taniguchi, Naoyuki and Daigo, Yataro and Nakamura, Yusuke and Hayashi, Norio and others},
         journal={Gastroenterology},
         volume={137},
         number={1},
         pages={188--198},
         year={2009},
         publisher={Elsevier}
}
@article{guo2013detection,
         title={Detection of hypermethylated fibrillin-1 in the stool samples of colorectal cancer patients},
         author={Guo, Qi and Song, Yongchun and Zhang, Hao and Wu, Xuandi and Xia, Peng and Dang, Chengxue},
         journal={Medical Oncology},
         volume={30},
         number={4},
         pages={1--5},
         year={2013},
         publisher={Springer}
}
@article{ouderkirk2014non,
         title={Non-muscle myosins in tumor progression, cancer cell invasion, and metastasis},
         author={Ouderkirk, Jessica L and Krendel, Mira},
         journal={Cytoskeleton},
         volume={71},
         number={8},
         pages={447--463},
         year={2014},
         publisher={Wiley Online Library}
}
@article{rochester2005silencing,
  title={Silencing of the IGF1R gene enhances sensitivity to DNA-damaging agents in both PTEN wild-type and mutant human prostate cancer},
  author={Rochester, Mark A and Riedemann, Johann and Hellawell, Giles O and Brewster, Simon F and Macaulay, Valentine M},
  journal={Cancer gene therapy},
  volume={12},
  number={1},
  pages={90--100},
  year={2005},
  publisher={Nature Publishing Group}
}
@article{thermes2006medaka,
         title={Medaka simplet (FAM53B) belongs to a family of novel vertebrate genes controlling cell proliferation},
         author={Thermes, Violette and Candal, Eva and Alunni, Alessandro and Serin, Guillaume and Bourrat, Franck and Joly, Jean-St{\'e}phane},
  journal={Development},
  volume={133},
  number={10},
  pages={1881--1890},
  year={2006},
  publisher={The Company of Biologists Ltd}
}
@article{chan2001molecular,
  title={Molecular cloning and characterization of a RING-H2 finger protein, ANAPC11, the human homolog of yeast Apc11p},
  author={Chan, Anna H and Lee, Simon MY and Chim, Stephen S and Kok, Louis DS and Waye, Mary MY and Lee, Cheuk-Yu and Fung, Kwok-Pui and Tsui, Stephen KW},
  journal={Journal of cellular biochemistry},
  volume={83},
  number={2},
  pages={249--258},
  year={2001},
  publisher={Wiley Online Library}
}
@article{xie2013larp1,
         title={LARP1 predict the prognosis for early-stage and AFP-normal hepatocellular carcinoma},
         author={Xie, Chan and Huang, Li and Xie, Shibin and Xie, Dongying and Zhang, Genlin and Wang, Peipei and Peng, Liang and Gao, Zhiliang},
         journal={Journal of translational medicine},
         volume={11},
         number={1},
         pages={1},
         year={2013},
         publisher={BioMed Central}
}
@article{agathanggelou2001methylation,
  title={Methylation associated inactivation of RASSF1A from region 3p21. 3 in lung, breast and ovarian tumours},
  author={Agathanggelou, Angelo and Honorio, Sofia and Macartney, Donia P and Martinez, Alonso and Dallol, Ashraf and Rader, Janet and Fullwood, Paul and Chauhan, Anita and Walker, Rosemary and Shaw, Jacqueline A and others},
  journal={Oncogene},
  volume={20},
  number={12},
  pages={1509--1518},
  year={2001}
}
@article{iliopoulos2005fragile,
         title={Fragile genes as biomarkers: epigenetic control of WWOX and FHIT in lung, breast and bladder cancer},
         author={Iliopoulos, Dimitrios and Guler, Gulnur and Han, Shuang-Yin and Johnston, Danika and Druck, Teresa and McCorkell, Kelly A and Palazzo, Juan and McCue, Peter A and Baffa, Raffaele and Huebner, Kay},
         journal={Oncogene},
         volume={24},
         number={9},
         pages={1625--1633},
         year={2005},
         publisher={Nature Publishing Group}
}
@article{cancer2014comprehensive,
  title={Comprehensive molecular profiling of lung adenocarcinoma},
  author={Cancer Genome Atlas Research Network and others},
  journal={Nature},
  volume={511},
  number={7511},
  pages={543--550},
  year={2014},
  publisher={Nature Publishing Group}
}
@article{fanarraga2010tbcd,
  title={TBCD links centriologenesis, spindle microtubule dynamics, and midbody abscission in human cells},
  author={Fanarraga, M{\'o}nica L{\'o}pez and Bellido, Javier and Ja{\'e}n, Cristina and Villegas, Juan Carlos and Zabala, Juan Carlos},
  journal={PloS one},
  volume={5},
  number={1},
  pages={e8846},
  year={2010},
  publisher={Public Library of Science}
}
@article{folgueira2005gene,
  title={Gene expression profile associated with response to doxorubicin-based therapy in breast cancer},
  author={Folgueira, Maria Aparecida Azevedo Koike and Carraro, Dirce Maria and Brentani, Helena and da Costa Patr{\~a}o, Diogo Ferreira and Barbosa, Edson Mantovani and Netto, M{\'a}rio Mour{\~a}o and Caldeira, Jos{\'e} Roberto F{\'\i}garo and Katayama, Maria Lucia Hirata and Soares, Fernando Augusto and Oliveira, C{\'e}lia Tosello and others},
  journal={Clinical Cancer Research},
  volume={11},
  number={20},
  pages={7434--7443},
  year={2005},
  publisher={AACR}
}
@article{montagna2003septin,
  title={The Septin 9 (MSF) gene is amplified and overexpressed in mouse mammary gland adenocarcinomas and human breast cancer cell lines},
  author={Montagna, Cristina and Lyu, Myung-Soo and Hunter, Kent and Lukes, Luanne and Lowther, William and Reppert, Tricia and Hissong, Bruce and Weaver, Zo{\"e} and Ried, Thomas},
  journal={Cancer research},
  volume={63},
  number={9},
  pages={2179--2187},
  year={2003},
  publisher={AACR}
}
@article{rakyan2011epigenome,
  title={Epigenome-wide association studies for common human diseases},
  author={Rakyan, Vardhman K and Down, Thomas A and Balding, David J and Beck, Stephan},
  journal={Nature Reviews Genetics},
  volume={12},
  number={8},
  pages={529--541},
  year={2011},
  publisher={Nature Publishing Group}
}
@article{breitling2011tobacco,
  title={Tobacco-smoking-related differential DNA methylation: 27K discovery and replication},
  author={Breitling, Lutz P and Yang, Rongxi and Korn, Bernhard and Burwinkel, Barbara and Brenner, Hermann},
  journal={The American Journal of Human Genetics},
  volume={88},
  number={4},
  pages={450--457},
  year={2011},
  publisher={Elsevier}
}
@article{van2011adaptive,
  title={The adaptive and the thresholded Lasso for potentially misspecified models (and a lower bound for the Lasso)},
  author={van de Geer, Sara and B{\"u}hlmann, Peter and Zhou, Shuheng and others},
  journal={Electronic Journal of Statistics},
  volume={5},
  pages={688--749},
  year={2011},
  publisher={The Institute of Mathematical Statistics and the Bernoulli Society}
}
@article{fraga2002dna,
  title={DNA methylation: a profile of methods and applications},
  author={Fraga, Mario F and Esteller, Manel},
  journal={Biotechniques},
  volume={33},
  number={3},
  pages={632--649},
  year={2002},
  publisher={EATON PUBLISHING}
}
@article{bibikova2009genome,
  title={Genome-wide DNA methylation profiling using Infinium{\textregistered} assay},
  author={Bibikova, Marina and Le, Jennie and Barnes, Bret and Saedinia-Melnyk, Shadi and Zhou, Lixin and Shen, Richard and Gunderson, Kevin L},
  year={2009},
  publisher={Future Medicine}
}
@article{pinkel1998high,
  title={High resolution analysis of DNA copy number variation using comparative genomic hybridization to microarrays},
  author={Pinkel, Daniel and Segraves, Richard and Sudar, Damir and Clark, Steven and Poole, Ian and Kowbel, David and Collins, Colin and Kuo, Wen-Lin and Chen, Chira and Zhai, Ye and others},
  journal={Nature genetics},
  volume={20},
  number={2},
  pages={207--211},
  year={1998},
  publisher={Nature Publishing Group}
}
@article{shlien2009copy,
  title={Copy number variations and cancer},
  author={Shlien, Adam and Malkin, David},
  journal={Genome medicine},
  volume={1},
  number={6},
  pages={1},
  year={2009},
  publisher={BioMed Central}
}
@article{troyanskaya2001missing,
  title={Missing value estimation methods for DNA microarrays},
  author={Troyanskaya, Olga and Cantor, Michael and Sherlock, Gavin and Brown, Pat and Hastie, Trevor and Tibshirani, Robert and Botstein, David and Altman, Russ B},
  journal={Bioinformatics},
  volume={17},
  number={6},
  pages={520--525},
  year={2001},
  publisher={Oxford Univ Press}
}
@article{figueroa2010dna,
  title={DNA methylation signatures identify biologically distinct subtypes in acute myeloid leukemia},
  author={Figueroa, Maria E and Lugthart, Sanne and Li, Yushan and Erpelinck-Verschueren, Claudia and Deng, Xutao and Christos, Paul J and Schifano, Elizabeth and Booth, James and van Putten, Wim and Skrabanek, Lucy and others},
  journal={Cancer cell},
  volume={17},
  number={1},
  pages={13--27},
  year={2010},
  publisher={Elsevier}
}
@article{van2010array,
  title={Array-based DNA methylation profiling for breast cancer subtype discrimination},
  author={Van der Auwera, Ilse and Yu, Wayne and Suo, Liping and Van Neste, Leander and Van Dam, Peter and Van Marck, Eric A and Pauwels, Patrick and Vermeulen, Peter B and Dirix, Luc Y and Van Laere, Steven J},
  journal={PLoS One},
  volume={5},
  number={9},
  pages={e12616},
  year={2010},
  publisher={Public Library of Science}
}
@article{nilsen2012copynumber,
  title={Copynumber: Efficient algorithms for single-and multi-track copy number segmentation},
  author={Nilsen, Gro and Liest{\o}l, Knut and Van Loo, Peter and Vollan, Hans Kristian Moen and Eide, Marianne B and Rueda, Oscar M and Chin, Suet-Feung and Russell, Roslin and Baumbusch, Lars O and Caldas, Carlos and others},
  journal={BMC genomics},
  volume={13},
  number={1},
  pages={591},
  year={2012},
  publisher={BioMed Central Ltd}
}
@Manual{imputer,
    title = {impute: impute: Imputation for microarray data},
    author = {Trevor Hastie and Robert Tibshirani and Balasubramanian Narasimhan and Gilbert Chu},
    note = {R package version 1.40.0},
  }

@article{yendamuri2007tumor,
  title={Tumor suppressor functions of ARLTS1 in lung cancers},
  author={Yendamuri, Sai and Trapasso, Francesco and Ferracin, Manuela and Cesari, Rossano and Sevignani, Cinzia and Shimizu, Masayoshi and Rattan, Shashi and Kuroki, Tamotsu and Dumon, Kristoffel R and Bullrich, Florencia and others},
  journal={Cancer research},
  volume={67},
  number={16},
  pages={7738--7745},
  year={2007},
  publisher={AACR}
}
@article{benjamini1995controlling,
  title={Controlling the false discovery rate: a practical and powerful approach to multiple testing},
  author={Benjamini, Yoav and Hochberg, Yosef},
  journal={Journal of the royal statistical society. Series B (Methodological)},
  pages={289--300},
  year={1995},
  publisher={JSTOR}
}
@article{esteller2001gene,
  title={A gene hypermethylation profile of human cancer},
  author={Esteller, Manel and Corn, Paul G and Baylin, Stephen B and Herman, James G},
  journal={Cancer research},
  volume={61},
  number={8},
  pages={3225--3229},
  year={2001},
  publisher={AACR}
}
@article{welter2014nhgri,
  title={The NHGRI GWAS Catalog, a curated resource of SNP-trait associations},
  author={Welter, Danielle and MacArthur, Jacqueline and Morales, Joannella and Burdett, Tony and Hall, Peggy and Junkins, Heather and Klemm, Alan and Flicek, Paul and Manolio, Teri and Hindorff, Lucia and others},
  journal={Nucleic acids research},
  volume={42},
  number={D1},
  pages={D1001--D1006},
  year={2014},
  publisher={Oxford Univ Press}
}
@Manual{spaccr,
	title={SpaCCr: A package for genomic region detection via spatial convex clustering.},
	author={John Nagorski},
	note={R package version 0.1.0},
}

















































